Smooth optimization using global and local low-rank regularizers

Many inverse problems and signal processing problems involve low-rank regularizers based on the nuclear norm. Commonly, proximal gradient methods (PGM) are adopted to solve this type of non-smooth problems as they can offer fast and guaranteed convergence. However, PGM methods cannot be simply applied in settings where low-rank models are imposed locally on overlapping patches; therefore, heuristic approaches have been proposed that lack convergence guarantees. In this work we propose to replace the nuclear norm with a smooth approximation in which a Huber-type function is applied to each singular value. By providing a theoretical framework based on singular value function theory, we show that important properties can be established for the proposed regularizer, such as: convexity, differentiability, and Lipschitz continuity of the gradient. Moreover, we provide a closed-form expression for the regularizer gradient, enabling the use of standard iterative gradient-based optimization algorithms (e.g., nonlinear conjugate gradient) that can easily address the case of overlapping patches and have well-known convergence guarantees. In addition, we provide a novel step-size selection strategy based on a quadratic majorizer of the line-search function that leverages the Huber characteristics of the proposed regularizer. Finally, we assess the proposed optimization framework by providing empirical results in dynamic magnetic resonance imaging (MRI) reconstruction in the context of local low-rank models with overlapping patches.

==> def,eps.tex <==
% def,eps.tex
% Latex2e macros for including Encapsulated Postscript (.eps)
% /opt/gnu/tex/doc/user/grfguide.ps
% Needs: \usepackage[dvips,draft]{graphicx}
% Picture: \ineps{dir}{file}{size}
% Centered picture: \inceps{dir}{file}{size}
% Captioned figure: \figeps[htbp]{dir}{file}{size}{caption}
% Centered lr picture: \incepslr{dir}{file1}{file2}{size}
% Captioned lr figure: \figepslr[htbp]{dir}{file1}{file2}{size}{caption}
% Centered quad figure:
%	\figepsquad{size}{dir}{file1}{file2}{file3}{file4}{caption}
% "file" does not include the .eps, and also becomes the figure label.
% "size" is typically Esize.  optional argument specifies position
% note: the graphicx package has a command that can specify order of
% suffixes to try: \DeclareGraphicsExtensions{.eps,.pdf}
%
\ifx \ecaption \undefined
	\newcommand{\ecaption}{\caption}
\fi

%
% \inps{width=}{size}{dir}{root}{suffix}
%
\providecommand{\figcent}[1]		{\mbox{}\hfill#1\hfill\mbox{}}
%\providecommand{\figsuffix}		{.eps}
\providecommand{\figsuffix}		{}
\providecommand{\figsuffixc}		{.epsc}
\providecommand{\inps}[5]		{\includegraphics[#1#2]{#3/#4#5}}
\providecommand{\ineps}[4][width=]	{\inps{#1}{#4}{#2}{#3}{\figsuffix}}
\providecommand{\inepsc}[4][width=]	{\inps{#1}{#4}{#2}{#3}{\figsuffixc}}
\providecommand{\inceps}[4][width=]	{\figcent{\ineps[#1]{#2}{#3}{#4}}}
\providecommand{\inpdf}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.pdf}}
\providecommand{\injpg}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.jpg}}
\providecommand{\intga}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.tga}}
\providecommand{\flabel}[1]		{\label{#1}} % figure label

% captioned/labeled eps, for use within a multiple-plot floating figure
\providecommand{\capeps}[4]{% dir file width caption
\inceps{#1}{#2}{#3}%
\ecaption{#4}%
\flabel{#2}}

\providecommand{\figeps}[5][htbp]{%
\begin{figure}[#1]%
\capeps{#2}{#3}{#4}{#5}%
\end{figure}}

\providecommand{\figepsc}[5][htbp]{%
\begin{figure}[#1]%
\figcent{\inepsc{#2}{#3}{#4}}%
\ecaption{#5}%
\flabel{#3}%
\end{figure}}

\providecommand{\figepsstar}[5][htbp]{%
\begin{figure*}[#1]%
\inceps{#2}{#3}{#4}%
\ecaption{#5}%
\flabel{#3}%
\end{figure*}}

%
% for 2 side-by-side
%

%
% Centered lr picture: \incepslr{dir}{file1}{file2}{size}
\providecommand{\incepslr}[4]{%
\lfill\ineps{#1}{#2}{#4}\hfill\ineps{#1}{#3}{#4}\rfill}

%
% Captioned lr figure: \figepslr[htbp]{dir}{file1}{file2}{size}{caption}
%
\providecommand{\figepslr}[6][htbp]{%
\begin{figure}[#1]%
\incepslr{#2}{#3}{#4}{#5}%
\ecaption{#6}%
\flabel{#3}%
\flabel{#4}%
\end{figure}}

%
% captioned 4 as 2by2
%

%
% Captioned quad figure:
% \figepsquad[htbp]{size}{dir}{file1}{file2}{file3}{file4}{caption}
\providecommand{\figepsquad}[8][htbp]{%
\begin{figure}[#1]%
\incepslr{#3}{#4}{#5}{#2}%
\\%
\incepslr{#3}{#6}{#7}{#2}%
\ecaption{#8}%
\flabel{#4}\flabel{#5}\flabel{#6}\flabel{#7}%
\end{figure}}


==> def,gen.tex <==
% def,gen.tex
% Latex2e general macros
% Jeff Fessler

% sections
%\providecommand{\dirtex}		{/n/ir7/y/fessler/tex}
%\providecommand{\dirtex}		{.} % use TEXINPUTS instead
\providecommand{\inputtex}[1]		{\label{#1}\input{#1}}
\providecommand{\isection}[2]		{\section{#1}\inputtex{#2}}
\providecommand{\isubsection}[2]	{\subsection{#1}\inputtex{#2}}

% latin
%\providecommand{\etal}		{\emph{et al\@.}\xspace}
\providecommand{\etal}		{et al\@.\xspace}
\providecommand{\ie}		{\emph{i.e\@.}\xspace}
\providecommand{\eg}		{\emph{e.g\@.}\xspace}
\providecommand{\cf}		{\emph{cf\@.}\xspace}
\providecommand{\defacto}	{\emph{de facto}\xspace}
\providecommand{\adhoc}		{\emph{ad hoc}\xspace}
\providecommand{\apriori}	{\emph{a priori}\xspace}

% web
%\providecommand{\myurl}[1][]	{\texttt{http://web.eecs.umich.edu/$\sim$fessler#1}\xspace}
\providecommand{\myurlold}[1][]	{\texttt{web.eecs.umich.edu/$\sim$fessler#1}\xspace}
\providecommand{\myurl}[1][]	{\url{http://web.eecs.umich.edu/~fessler#1}\xspace}
\providecommand{\myweb}		{\url{http://web.eecs.umich.edu/~fessler}\xspace}
\providecommand{\onweb}[1]	{Available from \myweb.}


% comments environments
% when using \usepackage{verbatim},
% the following allows this: \begin{comments} ... \end{comments} 
\let\comments=\comment
\let\endcomments=\endcomment

% huge comments.
% unfortunately this bashes the \begin{comment} environment in verbatim.sty
% which is why i have defined the preceding \comments environment.
\long\def\comment#1{}
\providecommand{\uncomment}[1]	{#1}


% common environments
\providecommand{\bcent}		{\begin{center}}
\providecommand{\ecent}		{\end{center}}
\providecommand{\benum}		{\begin{enumerate}}
\providecommand{\eenum}		{\end{enumerate}}
\providecommand{\bitem}		{\begin{itemize}}
\providecommand{\eitem}		{\end{itemize}}
\providecommand{\bvers}		{\begin{verse}}
\providecommand{\evers}		{\end{verse}}
\providecommand{\btab}		{\begin{tabbing}}	% use \= and \>
\providecommand{\etab}		{\end{tabbing}}
%\providecommand{\bverb}	{\begin{verbatim}}
%\providecommand{\everb}	{\end{verbatim}}

% positioning
\providecommand{\lfill}		{\mbox{}\hfill}
\providecommand{\rfill}		{\hfill\mbox{}}
\newcommand{\cent}[1]		{\lfill{#1}\rfill}
\newcommand{\adjustfullwidth}[1] {\adjustbox{width=\linewidth}{#1}}

% box with text stacked up in it
%\newcommand{\stacktext}[2][c]	{\begin{tabular}{#1}#2\end{tabular}}
\DeclareRobustCommand{\stacktext}[2][c]	{\begin{tabular}{#1}#2\end{tabular}}
\newcommand{\fsbox}[2][c]	{\fbox{\stacktext[#1]{#2}}}

\providecommand{\ul}[1]		{\underline{#1}}
\providecommand{\ebox}[1]	{\mbox{\fbox{$\displaystyle#1$}}}
\providecommand{\cbox}[1]	{\[\ebox{#1}\]}

\providecommand{\makeboxc}[2] {\makebox[#1\linewidth][c]{#2}}

% top-aligned side-by-side mini-pages
\newcommand{\minipaget}[2] {% width1 box1
\begin{minipage}[t]{#1\linewidth}\vspace*{0pt}#2\end{minipage}}
\newcommand{\minipagett}[4] {% width1 width2 box1 box2
\minipaget{#1}{#3}\hfill\minipaget{#2}{#4}}
\newcommand{\minipagettt}[6] {% width1 width2 width3 box1 box2 box3
\minipaget{#1}{#4}\hfill\minipaget{#2}{#5}\hfill\minipaget{#3}{#6}}

% bullet list with normal spacing
\newcounter{blist}
\providecommand{\blistmark}	{\makebox[0pt]{$\bullet$}}
\providecommand{\blistitemsep}	{0pt}
\providecommand{\blist}[1][]	{%
\begin{list}{\blistmark}{%
\usecounter{blist}%
\setlength{\itemsep}{\blistitemsep}%
\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}%
\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{1.2em}%
\setlength{\labelsep}{0.5\leftmargin}% centers label in margin
\setlength{\labelwidth}{0em}%
#1}% user over-rides
}
\providecommand{\elist}		{\end{list}}
\providecommand{\elistup}	{\elist\vspace{-\parskip}} % no space after

% enum list with normal spacing
%\providecommand{\bcolor}[1] {#1}
\providecommand{\blistitemsep}	{0pt}
\providecommand{\bjfenum}[1][]	{%
\begin{list}{\bcolor{\arabic{blist}.} }{%
\usecounter{blist}%
\setlength{\itemsep}{\blistitemsep}%
\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}%
\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{0.0em}%
\setlength{\labelsep}{1.0\leftmargin}% label in margin?
\setlength{\labelwidth}{0pt}%
#1}% user over-rides
}

% Alpha list with normal spacing
\newcounter{blistAlph}
\providecommand{\blistAlph}[1][]
{\begin{list}{\makebox[0pt][l]{\Alph{blistAlph}.}}{%
\usecounter{blistAlph}%
\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{1.2em}%
\setlength{\labelsep}{1.0\leftmargin}% letter at left side of margin
\setlength{\labelwidth}{0.0\leftmargin}#1}%
}

% Roman list with a bit of spacing
\newcounter{blistRoman}
\providecommand{\blistRoman}[1][]
{\begin{list}{\Roman{blistRoman}.}{%
\usecounter{blistRoman}%
\setlength{\itemsep}{0.5em}\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{4em}%
\setlength{\labelsep}{0.4\leftmargin}
\setlength{\labelwidth}{0.6\leftmargin}#1}%
}

%
% Portrait
% use \pagesize[.2in]{5in}{7in} to center width and height
% first argument is optional parindent
% at top of page: 1in, \topmargin, \headheight(for header), \headsep
%
\providecommand{\myheadheight}	{0in}
\providecommand{\myheadsep}	{0in}
\providecommand{\Halfheight}	{5.5in}		% half of 11" vertical page
\providecommand{\Halfwidth}	{4.25in}	% half of 8.5" horizontal page
\providecommand{\pagesize}[3][\parindent]{
\setlength{\parindent}{#1}
\setlength{\textwidth}{#2}
\setlength{\textheight}{#3}
\setlength{\headsep}{\myheadsep}
\setlength{\headheight}{\myheadheight}
\setlength{\oddsidemargin}{\Halfwidth}
\addtolength{\oddsidemargin}{-0.5\textwidth}
\addtolength{\oddsidemargin}{-1in}
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\topmargin}{\Halfheight}
\addtolength{\topmargin}{-0.5\textheight}
\addtolength{\topmargin}{-0.5\headheight}
\addtolength{\topmargin}{-0.5\headsep}
\addtolength{\topmargin}{-1in}
}

%
% Landscape
% use \pagesizeland[.2in]{5in}{7in} to center width and height
% first argument is optional parindent
%
\providecommand{\pagesizeland}[3][\parindent]{
\setlength{\parindent}{#1}
\setlength{\textwidth}{#2}
\setlength{\textheight}{#3}
\setlength{\headsep}{0.0in}
\setlength{\headheight}{0.0in}
\setlength{\oddsidemargin}{5.5in}
\addtolength{\oddsidemargin}{-0.5\textwidth}
\addtolength{\oddsidemargin}{-1in}
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\topmargin}{4.25in}
\addtolength{\topmargin}{-0.5\textheight}
\addtolength{\topmargin}{-1in}
}

%
% half of top margin for headings.
%
\providecommand{\pagehead}{%
\setlength{\headsep}{\topmargin}%
\addtolength{\headsep}{1in}%
\setlength{\headsep}{0.5\headsep}%
\setlength{\headheight}{\headsep}%
\setlength{\topmargin}{-1in}%
}


==> def,math.tex <==
% def,math.tex
% latex2e definitions of math symbols

% todo: to fix fonts see http://tug.org/fonts/fontinstall.html
%\usepackage{bbm} % black-board math
%\providecommand{\jfbbm}[1]	{\xmath{\mathbbm{#1}}} % needs bbm package
%\providecommand{\jfbbm}[1]	{\xmath{\mathsf{#1}}} % todo: while bbm broken
\providecommand{\jfbbm}[1]	{\xmath{\mathbb{#1}}}

\providecommand{\qed}[1][0pt]	{\hfill\raisebox{#1}{\inmath{\Box}}} % need latexsym package
% the next command is my favorite way to define bold letters.
% it requires \usepackage{bm,jf-fun}
\providecommand{\blmath}[1]	{\jfunl{\bm{#1}}}	% bm, jf-fun

% symbols that might need defined in a symbol table
\providecommand{\bigone}[1][\Large]	{\mbox{ {#1 1}}\xspace}
%\providecommand{\indic}[2][\large]	{\xmath{\mbox{{#1 $1$}}_{\braces{#2}}}}
% another option for \indic would be \iota (or \rchi in jf-all.sty)
\providecommand{\indic}[2][]	{\xmath{\jfbbm{I}_{\braces{#2}}}}

%\providecommand{\reals}	{\xmath{\mathrm{I\kern-.2em R}}}
\providecommand{\reals}		{\jfbbm{R}}

\providecommand{\thus}		{\xmath{\stackrel{\textstyle .}{..}}}
\providecommand{\suchthat}	{\textnormal{ s.t. }}
\providecommand{\defequ}	{\stackrel{\bigtriangleup}{=}}
\providecommand{\iid}		{\stackrel{iid}{\sim}}
\providecommand{\icomplex}	{\xmath{\imath}}

\providecommand{\norm}[1]	{\xmath{\left\| #1 \right\|}}
\providecommand{\normr}[1]	{\xmath{\| #1 \|}}
\providecommand{\normb}[1]	{\xmath{\Big\| #1 \Big\|}}
\providecommand{\normbb}[1]	{\xmath{\Bigg\| #1 \Bigg\|}}
\providecommand{\floor}[1]	{\xmath{\left\lfloor #1 \right\rfloor}}
\providecommand{\ceil}[1]	{\xmath{\left\lceil #1 \right\rceil}}
%\providecommand{\inprod}[2]	{\xmath{\langle #1,\, #2 \rangle}}
\providecommand{\inprod}[2]	{\xmath{\mathop{\langle #1,\, #2 \rangle}\nolimits}}
\providecommand{\Inprod}[2]	{\xmath{\left\langle #1,\ #2 \right\rangle}}
\providecommand{\musec}		{\xmath{\mu\mathrm{sec}}}

% \modo: ordinary modulo with a bit of space: "x mod y"
\providecommand{\modo}[2]	{\xmath{#1 \mathop{\mathrm{mod}}\nolimits #2}}
% \modp: modulo with the first part in paren: "(x) mod y"
\providecommand{\modp}[2]	{\modo{(#1)}{#2}}
% \pmod: defined in amsmath to do (x mod y)


\let\equivsave\equiv
\def\equiv{\xmath{\equivsave}}

% notes
% amsmath has subscript stacking: \sum_{\substack{ n=1 \\ n \neq m}}^N
% dvips -Ppdf for making pdf files?  \special for pdf hyperlinks?

\providecommand{\sumstack}[2]	{\sum_{\substack{#1 \\ #2}}}
\providecommand{\sumno}	{\sum\nolimits}

\providecommand{\ba}[1]		{\left[ \begin{array}{#1}}
\providecommand{\ea}		{\end{array} \right]}
\providecommand{\be}		{\begin{equation}}
\providecommand{\ee}[1]		{\label{#1}\end{equation}}
\providecommand{\den}[2]	{\begin{equation} #1 \label{#2} \end{equation}}
\providecommand{\bea}		{\begin{eqnarray}}
\providecommand{\eea}[1]	{\label{#1}\end{eqnarray}}
\providecommand{\beas}		{\begin{eqnarray*}} % obsolete! use desa{}
\providecommand{\eeas}		{\end{eqnarray*}} % obsolete!
%\providecommand{\bels}		{\begin{align*}} % requires amsmath
%\providecommand{\eels}		{\end{align*}}
%\providecommand{\bels}		{\begin{align*}} % requires amsmath
\providecommand{\beals}[1][1]	{\begin{alignat*}{#1}} % requires amsmath
\providecommand{\eeals}		{\end{alignat*}}

% displayed but un-numbered (*'d) equations using aligned
\providecommand{\desa}[1]	{\begin{align*} #1 \end{align*}} % amsmath
%\providecommand{\desa}[1]	{\begin{equation*}% % (pre 2022-11-20)
%	\begin{aligned}#1\end{aligned}\end{equation*}} % amsmath
% variant where first line is moved left using \MoveEqLeft from mathtools
\providecommand{\desal}[1]	{\begin{equation*}%
	\begin{aligned}\MoveEqLeft#1\end{aligned}\end{equation*}} % amsmath

% numbered versions (these number every line unless \nonum or \notag used)
\providecommand{\dena}[2]
	{\begin{align}#1\label{#2}\end{align}} % amsmath
\providecommand{\denal}[2]
	{\begin{align}\MoveEqLeft#1\label{#2}\end{align}} % amsmath

\providecommand{\denalt}[3]{ % text eqn label
\begin{flalign}
\text{#1} && #2 &&
\label{#3}
\end{flalign}
}

% obsolete: use desa and dena instead
\providecommand{\bals}		{\begin{equation*}\begin{aligned}} % amsmath
\providecommand{\eals}		{\end{aligned}\end{equation*}}
\providecommand{\beal}		{\begin{equation}\begin{aligned}[b]}
\providecommand{\eeal}[1]	{\end{aligned}\label{#1}\end{equation}}

% these do not work:
% http://tex.stackexchange.com/questions/3169/making-a-new-environment-combining-equation-and-split/3205#3205
%\providecommand{\bal}		{\begin{align}} % amsmath
%\providecommand{\eal}[1]	{\label{#1}\end{align}}
% but this works:
\providecommand{\bale}[2]	{\begin{align}#1\label{#2}\end{align}} % amsmath


% note: \ber and \eer and \bear are all dangerous it seems.
% use \berr and bearr instead!

%\providecommand{\ber}[1]	{\bgroup\renewcommand{\theequation}{#1}\be}
%\providecommand{\eer}[1]	{\label{#1}\end{equation}\egroup}
\providecommand{\berr}[2]{
\bgroup
\renewcommand{\theequation}{#1}
\be
#2
\ee{e,#1}
\egroup
\ignorespaces
}

%\providecommand{\bear}[1]	{\renewcommand{\theequation}{#1}\bea}
\providecommand{\bearr}[2]{
\bgroup
\renewcommand{\theequation}{#1}
\bea
#2
\eea{e,#1}
\egroup
\ignorespaces
}

% can this be done?
%\providecommand{\bebox}[1][\mbox{\fbox{$\displaystyle]	{\begin{equation}#1}
%\providecommand{\eebox}[1]	{$\}\}\label{#1}\end{equation}}
%\providecommand{\eebox}[2][$\}\}]	{#1\label{#2}\end{equation}}

\providecommand{\inmath}	{\ensuremath}
\providecommand{\xmath}[1]	{\inmath{#1}\xspace}
\providecommand{\bmath}[1]	{\xmath{\bm{#1}}}	% needs \usepackage{bm}
\providecommand{\eref}[1]	{(\protect\ref{#1})}
\providecommand{\fref}[2][]	{Fig.~\protect\ref{#2}#1}
\providecommand{\conj}		{\inmath{^*}}
%\providecommand{\conj}		{\inmath{^{\star}}}
\providecommand{\conjb}[1]	{\xmath{\brak{#1}\conj}} % [ ... ]^*
\providecommand{\degr}		{\xmath{^{\circ}}}
\providecommand{\isotop}[2]	{\inmath{^{#2}}#1\xspace}

\providecommand{\conv}		{\inmath{\ast}}
\providecommand{\cconv}		{\inmath{\ast\mbox{$\!\!$}\ast}}
\providecommand{\cconvsub}	{\inmath{\ast\mbox{$\!$}\ast}}
\providecommand{\ccconv}	{\inmath{\mathbin{\ast \mbox{$\!\!$} \ast \mbox{$\!\!$}\ast}}}

\providecommand{\inv}		{\inmath{^{-\!1}}}
\providecommand{\invT}		{\inmath{^{-\!\mathrm{T}}}}
\providecommand{\invH}		{\inmath{^{-\!\mathrm{H}}}}
\providecommand{\powten}[1]	{\inmath{\cdot10^{#1}}}
\providecommand{\uminus}	{\mathord{-}}

% invisible rule to make brackets etc. bigger
\providecommand{\irule}[1][-0.7em] {\rule[#1]{0pt}{0pt}}

\providecommand{\evalat}[2]	{\left. #1 \right|_{#2}}
\providecommand{\Evalat}[3][0.7em]
	{\left. #2 \irule[-#1] \right|_{#3}}	% -0.4\baselineskip
\providecommand{\choos}[3][-0.2]
% {\xmath{\fbox{\xmath{\begin{array}{c} #2\\[#1em]#3 \end{array}}}}}
 {\xmath{\left(\begin{array}{c} #2\\[#1em]#3 \end{array}\right)}}
%\providecommand{\choos}[2]	{\xmath{\left(\stackrel{#1}{#2}\right)}}

% \parin is "mathinner" parentheses; leaves more space around nearby operations
\providecommand{\parin}[1]	{\xmath{\mathinner{\left(#1\right)}}}
\providecommand{\paren}[1]	{\xmath{\left(#1\right)}}
\providecommand{\parenb}[1]	{\xmath{\Big(#1\Big)}}
\providecommand{\parens}[1]	{\xmath{(#1)}}
%\providecommand{\of}[1]	{\!\left(#1\right)}
\providecommand{\of}[1]		{\mleft(#1\mright)}
\providecommand{\ofb}[1]	{\!\Big(#1\Big)}
\providecommand{\brak}[1]	{\xmath{\left[#1\right]}}
\providecommand{\brakleft}[1]	{\xmath{\left[#1\right.}}
\providecommand{\brakright}[1]	{\xmath{\left.#1\right]}}
\providecommand{\brakb}[1]	{\xmath{\Big[#1\Big]}}
\providecommand{\brakbb}[1]	{\xmath{\Bigg[#1\Bigg]}}
\providecommand{\braces}[1]	{\xmath{\left\{#1\right\}}}
\providecommand{\bracesb}[1]	{\xmath{\Big\{#1\Big\}}}
\providecommand{\bracesbb}[1]	{\xmath{\Bigg\{#1\Bigg\}}}
\providecommand{\abs}[1]	{\xmath{\left| #1 \right|}}
\providecommand{\absr}[1]	{\xmath{| #1 |}} % regular size
\providecommand{\absb}[1]	{\xmath{\Big| #1 \Big|}}
\providecommand{\absbb}[1]	{\xmath{\Bigg| #1 \Bigg|}}

\providecommand{\overtext}[2]	{\overbrace{#1}^{\mbox{#2}}}
%\providecommand{\undertext}[2]	{\underbrace{#1}_{\mbox{#2}}}
\DeclareRobustCommand{\undertext}[2] {\underbrace{#1}_{\mbox{#2}}}
%\providecommand{\understack}[2] {\undertext{#1}{\stacktext{#2}}}
\DeclareRobustCommand{\understack}[2] {\undertext{#1}{\stacktext{#2}}}

\providecommand{\dddot}[1]	{\inmath{#1^{(3)}}}
\providecommand{\ddddot}[1]	{\inmath{#1^{(4)}}}
\providecommand{\dsqrt}[1]	{\xmath{\sqrt{\displaystyle #1}}}

\providecommand{\xfrac}[2]	{\xmath{\frac{#1}{#2}}}
\providecommand{\Half}[1][1]	{\xfrac{#1}{2}}
\providecommand{\half}[1][1]	{\xmath{{\scriptstyle \frac{#1}{2}}}}
\providecommand{\Frac}[2]	{\xmath{{#1}/{#2}}}
\providecommand{\pfrac}[3][]	{\xmath{\!\paren{#1\frac{#2}{#3}}}}
\providecommand{\pFrac}[3][]	{\xmath{\!\paren{#1\Frac{#2}{#3}}}}
\providecommand{\dpfrac}[3][]	{\xmath{\!\paren{#1\dfrac{#2}{#3}}}}
%\providecommand{\dfrac}[2]	% conflicts with amstex
\def\dfrac#1#2{\xmath{\displaystyle\frac{#1}{#2}}}
\def\implies	{\xmath{\Longrightarrow}} % ams?

%\providecommand{\eexp}		{\xmath{\mathop{\mathrm{e}}\nolimits}}
\providecommand{\eexp}		{\xmath{\mathinner{\mathrm{e}}}}
\providecommand{\Expi}[1]	{\xmath{\eexp^{\icomplex #1}}}
\providecommand{\expi}[1]	{\xmath{\exp\of{\icomplex #1}}}
\providecommand{\Expni}[1]	{\xmath{\eexp^{-\icomplex #1}}}
\providecommand{\expni}[1]	{\xmath{\exp\of{-\icomplex #1}}}
\providecommand{\Expo}[1]	{\xmath{\eexp^{#1}}}
\providecommand{\expo}[1]	{\xmath{\exp\of{#1}}}
\providecommand{\Expn}[1]	{\xmath{\eexp^{-#1}}}
\providecommand{\expn}[1]	{\xmath{\exp\of{-#1}}}
\providecommand{\Exp}		{\expo}	% backward compat
\providecommand{\Cos}[1]	{\xmath{\cos\of{#1}}}
\providecommand{\Sin}[1]	{\xmath{\sin\of{#1}}}

%
% the following are all obsolete due to jf-fun.sty
%
\providecommand{\Normal}[1]	{{\mathcal N}\of{#1}}
\providecommand{\mathword}[3][]	{\,\inmath{\mathrm{#2}#1\of{#3}}}
\providecommand{\wordbrace}[3][]{\,\inmath{\mathrm{#2}#1\!\braces{#3}}}
\providecommand{\Poisson}[1]	{\wordbrace{Poisson}{#1}}
\providecommand{\diag}[1]	{\wordbrace{Diag}{#1}}
\providecommand{\var}[1]	{\wordbrace{Var}{#1}}
\providecommand{\cov}[1]	{\wordbrace{Cov}{#1}}
%\providecommand{\sinc}[2][]	{\mathword[#1]{sinc}{#2}}
\providecommand{\sinc}		{\Ofun{\mathrm{sinc}}}
\providecommand{\rect}[1] 	{\mathword{rect}{#1}}
\providecommand{\sgn}[1] 	{\mathword{sgn}{#1}}
\providecommand{\real}[1]	{\mathword{real}{#1}}
\providecommand{\imag}[1]	{\mathword{imag}{#1}}

\providecommand{\mystack}[2][c]	{\xmath{\begin{array}{#1} #2 \end{array}}}
\providecommand{\myvect}[2][c]	{\xmath{\brak{\mystack[#1]{#2}}}}
\providecommand{\mymat}[1]	{\xmath{\begin{bmatrix} #1 \end{bmatrix}}} % amsmath, up to 10 cols, does not require [ccc]
\DeclareRobustCommand{\pmymat}[1] {\xmath{\begin{bmatrix} #1 \end{bmatrix}}}
\providecommand{\mymatsmall}[1]	{\xmath{\left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}} % amsmath, up to 10 cols, does not require [ccc]
\providecommand{\mymato}[2][]	{\xmath{\begin{bmatrix}[#1] #2 \end{bmatrix}}}
\providecommand{\leftbrace}[2][ll]	{\left\{ \mystack[#1]{#2} \right.}
\providecommand{\zeroother}	{\\ 0, & \mathrm{otherwise}}

% integrals and derivatives
\providecommand{\negint}	{-\!\!\int\!}
\providecommand{\intinf}	{\int_{\!-\infty}^{\infty}}
\providecommand{\iintinf}	{\intinf\intinf}
\providecommand{\iint}		{\int\!\!\!\int}
\providecommand{\iiint}		{\int\!\!\!\int\!\!\!\int}
\providecommand{\iiiint}	{\int\!\!\!\int\!\!\!\int\!\!\!\int}
% caution: \der \xj_n must be \der{\xj_n} to work properly!
\providecommand{\der}[1]	{\xmath{\mathop{\mathrm{d}#1}\nolimits}}
%\providecommand{\der}		{\xmath{\mathop{\mathrm{d}}\nolimits}}
%\providecommand{\der}		{\xmath{\mathrm{d}}}
\providecommand{\dxy}		{\der{x}\der{y}}
\providecommand{\dxyz}		{\der{x}\der{y}\der{z}}

\providecommand{\ddt}[1][t]	{\xfrac{\der{}}{\der{#1}}}
\providecommand{\dder}[2]	{\xfrac{\der{}^{#2}}{\der{#1}^{#2}}}
\providecommand{\fpart}[2][]	{\xfrac{\partial #1}{\partial #2}}
\providecommand{\ffpart}[2][]	{\xfrac{\partial^2 #1}{\partial #2^2}}
\providecommand{\fffpart}[2][]	{\xfrac{\partial^3 #1}{\partial #2^3}}
\providecommand{\ffpartt}[2]	{\xfrac{\partial^2}{\partial #1 \; \partial #2}}
%\providecommand{\Part}[1]	{\frac{\partial}{\partial #1}}
%\providecommand{\Partt}[1]	{\frac{\partial^2}{\partial #1}}
%\providecommand{\Parttt}[1]	{\frac{\partial^3}{\partial #1}}

\providecommand{\Gam}		{\jfunl{\Gamma}}
\providecommand{\eps}		{\jfunl{\epsilon}}
\providecommand{\veps}		{\jfunl{\varepsilon}}


% https://tex.stackexchange.com/questions/451786/how-do-i-put-a-circle-around-a-symbol
% ostar for circular convolution
\makeatletter
\newcommand{\ostar}{\mathbin{\mathpalette\make@circled\star}}
\newcommand{\make@circled}[2]{%
 \ooalign{$\m@th#1\smallbigcirc{#1}$\cr\hidewidth$\m@th#1#2$\hidewidth\cr}%
}
\newcommand{\smallbigcirc}[1]{%
 \vcenter{\hbox{\scalebox{0.77778}{$\m@th#1\bigcirc$}}}%
}
\makeatother

